HCL-TAT: A Hybrid Contrastive Learning Method for Few-shot Event Detection with Task-Adaptive Threshold

Conventional event detection models under supervised learning settings suffer from the inability of transfer to newly-emerged event types owing to lack of sufficient annotations. A commonly-adapted solution is to follow a identify-then-classify manner, which first identifies the triggers and then converts the classification task via a few-shot learning paradigm. However, these methods still fall far short of expectations due to: (i) insufficient learning of discriminative representations in low-resource scenarios, and (ii) trigger misidentification caused by the overlap of the learned representations of triggers and non-triggers. To address the problems, in this paper, we propose a novel Hybrid Contrastive Learning method with a Task-Adaptive Threshold (abbreviated as HCLTAT), which enables discriminative representation learning with a two-view contrastive loss (support-support and prototype-query), and devises a easily-adapted threshold to alleviate misidentification of triggers. Extensive experiments on the benchmark dataset FewEvent demonstrate the superiority of our method to achieve better results compared to the state-of-the-arts. All the code and data of this paper will be available for online public access.

==> EMNLP 2022/sections/abstract.tex <==
\maketitle
\begin{abstract}
  %Event detection (ED) is a key sub-task for event extraction in information extraction domain, which aims to identify triggers and categorize event mentions. Existing ED approaches have achieved promising results by following a paradigm of fine-tuning on pre-trained language models (PLMs). However, there exists a natural gap between PLMs and the fine-tuned ED model, which thus results in poor margin problem as the learned representations of event mentions are inadequate for discrimination, especially when the large majority of sampling instances in each batch are non-triggers. To overcome the problem, in this paper we propose a novel prototypical contrastive learning method named PCED, consisting of two components, namely dynamic prototype update (DPU) and distance-based loss re-weighting (DISLRE). Specifically, PCED is capable of fully exploiting label information in a supervised manner to enhance the discriminativeness of the learnt representation of event mentions, and then improve the performance of ED by making triggers and the prototype of the same class compact, and the remaining ones of different classes separable. Experiments on two widely used datasets ACE2005 and MAVEN demonstrate the superiority of our method to learn more meaningful representations and achieve better results compared to the state-of-the-arts. All the data and codes will be available to facilitate future research.
  
Conventional event detection models under supervised learning settings suffer from the inability of transfer to newly-emerged event types owing to lack of sufficient annotations. A commonly-adapted solution is to follow a identify-then-classify manner, which first identifies the triggers and then converts the classification task via a few-shot learning paradigm. However, these methods still fall far short of expectations due to:  (i) insufficient learning of discriminative representations in low-resource scenarios, and (ii) trigger misidentification caused by the overlap of the learned representations of triggers and non-triggers. To address the problems, in this paper, we propose a novel \textbf{\underline{H}}ybrid \textbf{\underline{C}}ontrastive \textbf{\underline{L}}earning method with a \textbf{\underline{T}}ask-\textbf{\underline{A}}daptive \textbf{\underline{T}}hreshold (abbreviated as HCL-TAT), which enables discriminative representation learning with a two-view contrastive loss (\textit{support-support} and \textit{prototype-query}), and devises an easily-adapted threshold to alleviate misidentification of triggers. Extensive experiments on the benchmark dataset FewEvent demonstrate the superiority of our method to achieve better results compared to the state-of-the-arts. All the code and data of this paper will be available for online public access.

  
\end{abstract} 

==> EMNLP 2022/sections/acknowledgement.tex <==
\section*{Acknowledgements}

This work was supported in part by the National Natural Science Foundation of China under Grant No.62276110, Grant No.61602197, Grant No.61772076, in part by CCF-AFSG Research Fund under Grant No.RF20210005, and in part by the fund of Joint Laboratory of HUST and Pingan Property \& Casualty Research (HPL). The authors would also like to thank the anonymous reviewers for their comments on improving the quality of this paper.

==> EMNLP 2022/sections/conclusion.tex <==
\section{Conclusion}

%By distinguishing ambiguous words better through a biased objective function, our model can integrate more information into the representation and disambiguate trigger words better. 
%This paper proposes a novel event detection model, Meta-ED, to combine a external-knowledge-enhanced trigger identifier with a label-enhanced meta-learning method to predict event types for words in a given sentence. By distinguishing ambiguous words better through a biased objective function, our model can integrate more information into the representation and disambiguate trigger words better. By exploiting a label-enhanced prototypical network, our model could further make accurate predictions for the specific event types. Experiments on ACE2005 dataset demonstrate the effectiveness of our approach, with improvement compared with the state-of-the-art model.

In this paper, we propose a contrastive learning method to make full use of limited data and produce more discriminative representations for FSED. Specifically, we first propose a hybrid contrastive loss, composed of support-support contrastive loss and prototype-query loss, to conduct supervised contrastive learning within support set and between support and query set respectively. Furthermore, we design a task-adaptive threshold method, to regularize the distance-based classifier in each episode. Experimental results show that by improving the representation learning and classifier learning simultaneously, our method boost the performance under all four settings on FewEvent dataset.

==> EMNLP 2022/sections/experiment.tex <==
%实验分为以下几个部分：实验设置（包括数据集介绍、验证方式介绍、实现细节）、baseline介绍、主要结果分析、消融实验分析、触发词检测子问题结果分析（按理说我们的方法对other分类效果更好的）、case study和降维图分析

\section{Experiments}

\subsection{Experimental Settings}

\paragraph{Dataset.} 
We conduct experiments on the newly-proposed largest few-shot event dataset \textbf{FewEvent}\footnote{https://github.com/231sm/Low\_Resource\_KBP} proposed by \cite{deng2020meta}. FewEvent contains more than 70000 event instances over 100 fine-grained event types, and is built from ACE2005, KBP2017 and external knowledge bases like Freebase and Wikipedia, thus it's representative and can take coverage of most event types. Following~\cite{cong2021PACRF}, we use the same 80 event types for training, 10 event types for validation and the rest 10 event types for testing, where event types between each subset are disjoint. The statistics of FewEvent dataset is listed in Appendix~\ref{sec:A}.


\paragraph{Evaluation.}
Same as previous works \cite{chen2015event}, we report micro precision, recall and F1 score over event types, among which F1 score is the most important metric. Following~\cite{cong2021PACRF}, we use the same episodic evaluation method to evaluate our model in few-shot settings, by randomly selecting episodes containing $N$-way-$K$-shot samples from the test set. We run each experiment 5 times to get the averages and standard deviations for fair comparison.

\paragraph{Implementation Details.}
We use bert-base-uncased model through huggingface's transformers\footnote{https://github.com/huggingface/transformers} to obtain the 768-dimensional token-level embeddings. Following~\cite{cong2021PACRF}, we also use episodic training and evaluation methods for few-shot event detection. In the training stage, we randomly select $N$-way-$K$-shot samples from training set for 20000 iterations. In each iteration, we first randomly select $N$ event types then assign $K$ instances for each type as the support set, and select other $M$ samples for each type as the query set. We manually tune the hyper-parameters by running similar $N$-way-$K$-shot episodic evaluation on the validation set for 1000 iterations, and the final test result is obtained by 3000 iterations on the test set. Since only 0.12\% of sentences are longer than 128, we set the maximum length to 128 and pad sentences shorter than 128 with a special character ``[PAD]''. We optimize our model using AdamW with a 1e-5 learning rate. For the contrastive learning part, the scalar temperature parameter $\tau$ is set to 0.5 and 0.1 for SSCL and PQCL, respectively, and the trade-off parameters of $\alpha$ and $\beta$ are both set to 0.5. We experiment with Pytorch 1.10 in Ubuntu 18.04. For 5-way-5-shot, 5-way-10-shot and 10-way-5-shot settings, we run the experiments on one NVIDIA GeForce RTX 2080 Ti. For 10-way-10-shot setting, we run the experiments on one NVIDIA GeForce RTX 3090.

\subsection{Baselines}

\begin{table*}[htb]
	\centering
	\scalebox{1.0}{
	\begin{tabular}{l|cccc}
		\toprule[1pt]
		\textbf{Model}    & \textbf{5-way-5-shot}    & \textbf{5-way-10-shot}    & \textbf{10-way-5-shot} & \textbf{10-way-10-shot}  \\
		\midrule
		LoLoss & 31.51 $\pm$ 1.56 & 31.70 $\pm$ 1.21 & 30.46 $\pm$ 1.38 & 30.32 $\pm$ 0.89 \\
		MatchLoss & 30.44 $\pm$ 0.99 & 30.68 $\pm$ 0.78 & 28.97 $\pm$ 0.61 & 30.05 $\pm$ 0.93 \\
		DMBPN   & 37.51 $\pm$ 2.60 & 38.14 $\pm$ 2.32 & 34.21 $\pm$ 1.45 & 35.31 $\pm$ 1.69 \\
		\midrule
		Proto-dot\dag & 41.54 $\pm$ 3.82 & 42.21 $\pm$ 0.68 & 33.27 $\pm$ 2.37 & 39.23 $\pm$ 2.95 \\
		Match\dag & 30.09 $\pm$ 1.71 & 48.10 $\pm$ 1.38 & 28.94 $\pm$ 1.15 & 45.91 $\pm$ 1.98 \\
		Proto\dag & 47.30 $\pm$ 2.55 & 54.81 $\pm$ 2.27 & 42.48 $\pm$ 1.00 & 50.14 $\pm$ 0.65 \\
		Vanilla CRF & 59.01 $\pm$ 0.81 & 62.21 $\pm$ 1.94 & 56.00 $\pm$ 1.51 & 59.35 $\pm$ 1.09 \\
		CDT & 59.30 $\pm$ 0.23 & 62.77 $\pm$ 0.12 & 56.41 $\pm$ 1.09 & 59.44 $\pm$ 1.83 \\
		PA-CRF & 62.25 $\pm$ 1.42 & 64.45 $\pm$ 0.49 & 58.48 $\pm$ 0.68 & 61.64 $\pm$ 0.81 \\
		\midrule
		\textbf{HCL-TAT}    & \textbf{66.96} $\pm$ 0.70 & \textbf{68.80} $\pm$ 0.85 & \textbf{64.19} $\pm$ 0.96 & \textbf{66.00} $\pm$ 0.81 \\
		\bottomrule[1pt]
	\end{tabular}}
    \caption{F1 scores ($10^{-2}$) of evaluated methods on FewEvent test set. \dag\, means the model is re-implemented by ourselves. The best scores are highlighted in boldface, with $p < 0.02$ under t-test.}
    \label{table_main_result}
\end{table*}

To comprehensively investigate the effectiveness of our method, we choose a variety of baselines on FewEvent, including two-stage methods and unified methods.

%We compare the proposed PCED with both data-driven and knowledge-driven baselines. \textbf{DMCNN}~\cite{chen2015event} and \textbf{JRNN}~\cite{nguyen2016joint} are traditional data-driven methods which employ CNN (with dynamic multi-pooling) and RNN respectively to extract events. \textbf{ANN-S2}~\cite{liu2017exploiting} exploits argument information to introduce supervised attention. \textbf{MOGANED}~\cite{yan2019event} and \textbf{GatedGCN}~\cite{lai-etal-2020-event} are both GNN-based models which incorporate syntactic knowledge, with hierarchical attention on multi-order graphs and gated mechanism, respectively. \textbf{RoBERTa} is a vanilla RoBERTa-based model, and \textbf{DMRoBERTa} is further equipped with dynamic multi-pooling to extract features, which is implemented by ourselves as a base model for the proposed method. \textbf{EKD}~\cite{tong2020improving} is a knowledge distillation framework which extracts open-domain trigger knowledge from external resources. The state-of-the-art ED model \textbf{CLEVE}~\cite{wang-etal-2021-cleve} enhances pre-training through contrastive learning on large-sclae unsupervised Wikipedia data. \textbf{EKD} and \textbf{CLEVE} both use Transformer-based PLMs as the encoder.

For \textbf{two-stage models}, we compare with \textbf{LoLoss}~\cite{lai2020exploiting}, \textbf{MatchLoss}~\cite{lai2020extensively} and \textbf{DMBPN}~\cite{deng2020meta}, by adding a trigger identification model before their methods. LoLoss uses matching information between examples in the support set as additional training signals, MatchLoss extends LoLoss to consider intra-cluster matching and inter-cluster information. DMBPN proposes the benchmark FSED dataset FewEvent, and proposes a dynamic memory network based model to preserve more contextual information for FSED.

For \textbf{unified models}, we compare with three typical few-shot classification baselines, \textbf{Proto-dot}, \textbf{Match} and \textbf{Proto}. Besides, we also compare with the state-of-the-art CRF-based methods, \textbf{Vanilla CRF}, \textbf{CDT}~\cite{hou-etal-2020-shot} and \textbf{PA-CRF}~\cite{cong2021PACRF}. Match, Proto and Proto-dot are similar metric-based model, with cosine similarity, euclidean distance and dot product used as metric respectively. We re-implement the three baselines since Cong ``[PAD]'' embeddings are used to calculate prototype of ``O'' type in previous work~\cite{cong2021PACRF}. Vanilla CRF adds a simple CRF layer behind baseline models, while CDT and PA-CRF exploits Gaussian distribution approximation and collapsed dependency transfer to enhance the CRF layer, respectively.


\subsection{Overall Performance}

We use Proto as the backbone model for HCL-TAT. Table \ref{table_main_result} show the overall performance on FewEvent test set. We can observe that: (i) Compared with two-stage models, unified models achieve much better results, which demonstrates the influence of error propagation and the advantage of unifed architectures. (ii) Among the three metric-based few-shot classification baselines, Proto achieves the best result. This indicates that euclidean distance is the best metric for FSED. Note that this 
observation conflicts with the conclusion in PA-CRF, because the authors uses ``[PAD]'' embeddings to calculate the prototype of ``O'' type. (iii) The re-implemented baselines have a lower performance compared with those in~\cite{cong2021PACRF}. This implies that when optimizing with only query-anchored loss, the model cannot learn discriminative representations and even using ``[PAD]'' embeddings to calculate the prototype of ``O'' type is a better choice than averaging the corresponding instance representations. (iv) Our proposed HCL-TAT achieves new state-of-the-art results under all four settings. Specifically, compared with PA-CRF, HCL-TAT brings an improvement of 4.71\%, 4.35\%, 5.71\% and 4.36\%, which proves the effectiveness of HCL-TAT to learn better representations and obtain better classification results. (v) Our proposed HCL-TAT achieve even higher results in 5-shot settings, which demonstrates the ability of HCL-TAT to make full use of limited data compared with other methods.

%(i) Our proposed PCED significantly outperforms various baseline methods. Compared with the base model DMRoBERTa and state-of-the-art method CLEVE, PCED brings an improvement of 3.3\%/0.9\% and 1.1\%/0.5\% on ACE2005/MAVEN respectively, which demonstrates the superiority of prototypical contrastive learning. (ii) PLM-based models (RoBERTa, DMRoBERTa, EKD, CLEVE and our PCED) outperform traditional neural-based models, demonstrating the effectiveness of pre-training knowledge in large-scale corpora. Besides, knowledge-driven methods have a better performance compared with vanilla data-driven methods, which shows the success of external knowledge even with the noise and semantic gap against ED. (iii) Compared with the state-of-the-art CLEVE, our PCED achieves competitive results without need for external resources and risk of introducing noise. We argue that this is due to the use of prototypical contrastive learning to generate more compact clusters in latent space and thus benefit more ambiguous triggers. 


\subsection{Ablation Study}

\begin{table*}[htb]
	\centering
	\scalebox{0.94}{
    \begin{tabular}{l|ccc|ccc}
        \toprule
        \multicolumn{1}{l|}{\multirow{2}*{\textbf{Model}}}      & \multicolumn{3}{c|}{\textbf{5-way-5-shot}} & \multicolumn{3}{c}{\textbf{5-way-10-shot}} \\
        \cmidrule{2-7}
        \multicolumn{1}{c|}{} & \textbf{P}       & \textbf{R}       & \textbf{F1}     & \textbf{P}       & \textbf{R}      & \textbf{F1}     \\
        \midrule
        HCL-TAT                 & \textbf{62.63} $\pm$ 2.31    & 72.04 $\pm$ 1.93    & \textbf{66.96} $\pm$ 0.70    & \textbf{63.87} $\pm$ 2.35       & 74.65 $\pm$ 1.36      & \textbf{68.80} $\pm$ 0.85      \\
        \;w/o SSCL                      & 59.61 $\pm$ 2.48       & 71.65 $\pm$ 1.72       & 65.03 $\pm$ 0.82       & 60.22 $\pm$ 4.78       & 74.38 $\pm$ 1.81      & 66.42 $\pm$ 2.34      \\
        \;w/o PQCL                      & 57.50 $\pm$ 1.80    & 71.88 $\pm$ 1.52    & 63.85 $\pm$ 0.67    & 60.88 $\pm$ 2.18    & 72.63 $\pm$ 1.23   & 66.21 $\pm$ 1.14   \\
        \;w/o HCL                      & 49.52 $\pm$ 4.34 & 74.67 $\pm$ 3.36 & 59.38 $\pm$ 2.59  & 57.72 $\pm$ 2.72   & 73.35 $\pm$ 1.10  & 64.57 $\pm$ 1.69  \\
        \;w/o TAT          & 46.69 $\pm$ 1.25       & \textbf{76.98} $\pm$ 0.29       & 58.12 $\pm$ 0.94       & 49.56 $\pm$ 1.11       & 76.33 $\pm$ 0.67      & 60.09 $\pm$ 0.92      \\
        \bottomrule
    \end{tabular}}
    \caption{Precision, recall and F1 scores ($10^{-2}$) of ablation study results on FewEvent test set. When remove both HCL and TAT, the method degenerates to a Proto model.}
    \label{table_ablation_study}
\end{table*}

%We further study the two main components in our model respectively, to prove whether these two models could interact well with help of external knowledge and label-enhanced prototypical networks.
We conduct ablation studies to investigate the effectiveness of each component in the proposed HCL-TAT model. The experimental results are shown in Table~\ref{table_ablation_study}.

\paragraph{Effect of Contrastive Learning.} We remove the two contrastive losses in HCL to observe the performance. We can conclude that: (i) When removing SSCL, the F1 score drops 1.93\%/2.38\% under 5-way-5-shot and 5-way-10-shot settings respectively, which indicates that SSCL could benefit the model by producing more separable representations for prototypes. (ii) When removing PQCL, the F1 scores drop by 3.11\%/2.59\%. This shows that compared with SSCL, PQCL contributes more to the improvement due to the information interaction between support and query set. Especially, in 5-way-10-shot-setting, the performance gap between SSCL and PQCL is slight, we believe the reason is that more instances in support set provide more training signals for SSCL. (iii) When removing both SSCL and PQCL, \ie HCL, the F1 scores drop significantly by 7.58\%/4.23\%, which proves the effectiveness of combining the two contrastive losses. Besides, we note that HCL achieves higher improvement in more difficult setting (5-shot), which further proves the superiority of HCL in few-shot scenarios. (iv) The improvement of HCL mainly comes from the improvement of precision score, which indicates that by producing more discriminative representations, HCL reduces the representation overlap between different types and thus alleviates the misidentification of triggers.

%Contrastive learning brings improvement on both datasets. Firstly, when removing the annotations, the standard UCL method which considers augmentations of the same instance as positives and all other instances as negatives still achieves better results, which proves the ability of contrastive learning to produce more discriminative representations. Secondly, with the introduction of label semantics, SCL further outperforms UCL and demonstrates the superiority of supervised contrastive learning to better utilize label information. Finally, PCL obtains even better results than SCL by contrasting instances with event prototypes. We attribute this to the ability of PCL to associate with all event types during training.

\paragraph{Effect of Task-adaptive Threshold.} To prove the effect of task-adaptive threshold (TAT), we remove this module and evaluate the performance under 5-way-5-shot and 5-way-10-shot settings. The results show that without TAT, the F1 scores drop dramatically by 8.84\%/8.71\%, in which the precision scores contribute most, with a 15.94\%/14.31\% decrease. This demonstrates that TAT could on the other hand eliminate the misidentification of triggers by regularizing the classification process.


\subsection{Performance of Trigger Identification}

\begin{table}[htb]
	\centering
	\scalebox{1.0}{
	\begin{tabular}{l|cc}
		\toprule[1pt]
		\textbf{Model}    & \textbf{FSTI}    & \textbf{FSED}  \\
		\midrule
		PA-CRF & 63.68 & 62.25  \\
		HCL-TAT & 68.18 & 66.96 \\
		\bottomrule[1pt]
	\end{tabular}}
    \caption{Average F1 scores ($10^{-2}$) of HCL-TAT and PA-CRF on FSTI and FSED tasks, on FewEvent test set under 5-way-5-shot setting.}
    \label{table_trigger_identification_result}
\end{table}

To investigate the effectiveness of our method to solve trigger identification problem, we compare the results between HCL-TAT and the state-of-the-art method PA-CRF. As shown in Table~\ref{table_trigger_identification_result}, HCL-TAT achieves 68.18\% on few-shot trigger identification (FSTI) task, bringing a +4.5\% improvement compared with PA-CRF. This indicates that the main improvement of HCL-TAT comes from more accurate identification of trigger words, which can be attributed to two aspects. First, HCL-TAT learns more discriminative representations for both support set and query set through hybrid contrastive learning. Second, the introduced task-adaptive threshold further regularizes the classification process to avoid misidentification.

\subsection{N-way-K-shot Evaluation}

\begin{figure}[htb]
    \centering
    \includegraphics[width=1.0\linewidth]{EMNLP 2022/figures/n-way-k-shot-evaluation.pdf}
    \caption{$N$-way-$K$-shot evaluations for three different models. The left part illustrates F1 scores in $N$-way-5-shot settings, and the right part illustrates F1 scores in 5-way-$K$-shot settings. We run each experiment once to analyze the tendency of F1 scores.}
    \label{fig:n-way-k-shot-evaluation}
\end{figure}

We conduct $N$-way-$K$-shot evaluation to investigate the performance tendency of different models in different few-shot settings. For fair comparison, we re-run PA-CRF with the released source code to obtain the results. As illustrated in Figure~\ref{fig:n-way-k-shot-evaluation}, generally, when the shot number $K$ is fixed, F1 scores tend to drop with the increase of way number $N$, and when the way number $N$ is fixed, F1 scores tend to improve with the increase of shot number $K$. Besides, we can observe that the backbone Proto model is more sensitive to the change of way and shot numbers, which indicates that the vanilla prototypical network is more vulnerable to limited data. Moreover, in all settings, HCL-TAT outperforms other methods with a large margin, especially when $N$ is large. This proves that our method shows more robustness to the way number with the help of HCL to fully exploit information between event types and produce more discriminative representations.

\subsection{Learning Visualization}

\begin{figure*}[htb]
	\centering
	\subfloat[Proto]{\label{fig:visual_proto}\includegraphics[width=0.25\linewidth]{EMNLP 2022/figures/proto_visualization.pdf}}
	\subfloat[Proto+SSCL]{\label{fig:visual_sscl}\includegraphics[width=0.25\linewidth]{EMNLP 2022/figures/sscl_visualization.pdf}}
	\subfloat[Proto+PQCL]{\label{fig:visual_pqcl}\includegraphics[width=0.25\linewidth]{EMNLP 2022/figures/pqcl_visualization.pdf}}
	\subfloat[Proto+HCL]{\label{fig:visual_hcl}\includegraphics[width=0.25\linewidth]{EMNLP 2022/figures/hcl_visualization.pdf}}\\
	\caption{Visualization of trigger embeddings in the same episode on FewEvent test set, under 5-way-10-shot setting. From left to right, the visualazation results of four FSED models are given respectively.}
	\label{fig:visual_all}
\end{figure*}

Given the same test episode, we use t-SNE to visualize the embeddings of triggers for the backbone model Proto with and without using contrast learning. From Figure~\ref{fig:visual_all}, we can observe that: (i) Proto achieves similar results as PA-CRF (see Figure~\ref{fig:visual_a}), with some instances hard to categorize. This proves that PA-CRF fails to improve representation learning by modeling label dependencies. (ii) SSCL and PQCL both contributes to the improvement of representations, while SSCL forms more compact clusters and PQCL learns more separable embedding space. (iii) When jointly using HCL, advantages of SSCL and PQCL are combined and more discriminative representations are produced to improve the performance. (iv) Besides, in Figure~\ref{fig:visual_hcl}, ``Fine'' and ``Arrest-Jail'', ``Nominate'' and ``Resignation'' have the common supertype ``Justice'' and ``Personnel'', respectively, and representations of event types belonging to the same supertype are relatively close. This shows that HCL automatically learns the relations between event types.

%\subsection{Learning Visualization\label{Sec: 4.7}}


%Contrastive learning naturally benefits representation learning by inducing more discriminative features. As illustrated in Figure \ref{fig:visual}, we visualize the representations learned by the state-of-the-art model PA-CRF and our proposed HCL-TAT respectively, to give an intuitive understanding of the learning process with and without the use of contrastive loss. We can observe that, when the model is trained with the query-anchored cross-entropy loss, the separation between event clusters becomes ambiguous, which corroborates with our discussion in Section~\ref{Sec: 1}. When contrastive loss is used, the overlap between event types is reduced, and representations of the same event type are formed into more compact clusters, so that the decision boundary becomes clearer. This proves the ability of HCL-TAT to learn more discriminative representations, which we argue is the dominating reason for performance improvement.


==> EMNLP 2022/sections/introduction.tex <==
%1. 交代研究任务（简单例子说明什么是触发词）和小样本场景下的挑战
%2. 交代目前解决小样本事件检测的方案（基于原型网络的度量元学习为基础），先将二阶段模型的问题，再讲crf改进类方案在事件检测中的缺陷，不要讲建模label dependency用处不大，而要说明crf的那种方式建模不好，以及忽略了O类
%3. 讲我们的思路。既然crf建模label dependency效果不好，那么我们需要对有限样本充分利用，学出更具区分性的表示。直观的想法是，support内部对比学习，但是这样只利用了support内的信息，而且优化方向不明，因此再提出以prototype为anchor的prototype-query对比学习。在此基础上，由于other类语义比较复杂多样，单靠对比学习可能仍然和事件类间存在overlap，所以我们提出用一个动态自适应阈值去控制分类过程，防止把一些other类样本预测成事件
%4. 较为详细地介绍方案。主要是两个对比学习loss的设计，以及动态与之的方案（先铺垫，强调这个阈值应该是task-adaptive的，再讲是用平均来计算的）
%5. 总结贡献（我们是第一个在小样本事件检测中提出这两种对比学习的联合使用，以同时提升prototype的质量和使query样本获得更高的语义相关度；此外就是阈值的设计来控制other类边界不清的问题，以及实验结果）

\section{Introduction\label{Sec: 1}}

Event detection (ED) is the subtask of information extraction (IE)~\cite{pan-etal-2021-context-aware,pan-etal-2021-noisy}, which aims at extracting events of task-specified types from an input text and is crucial for many downstream applications such as text summarization \cite{ge2016news} and machine reading comprehension \cite{qiu2019machine}. For example, in the sentence ``Kenyan police intensify manhunt for \textbf{\textit{terror}} suspects", an ideal ED model is to identify ``\textbf{\textit{terror}}'' as a trigger word and classify it into ``\textbf{Conflict.Attack}'' event type. Previous works commonly formulate ED as a token-level classification problem and follow a supervised manner~\cite{chen2015event,liu2017exploiting,nguyen2018graph,zhao2018document,wang-etal-2019-adversarial-training,tong2020improving}. Despite the promising results, in real-world scenarios, new event types are constantly emerging with only a few samples, which gives rise to the problem of low generation on newly-emerged event types, in view of insufficient annotated data. Therefore, it is reasonable to convert the traditional supervised-based event detection task to the few-shot event detection (FSED) problem. 

%Most FSED methods follow a paradigm of meta learning due to its wide application in few-shot learning tasks. Meta-learning, also known as ``learn to learn'', is inspired from the ability of humans to learn new knowledge from few instances. In this setting, the model is required to optimize with a number of sampled episodes during training, and learn to generalize to any unseen episode with only a few samples during testing. Each episode contains $N$ classes, and each class has $K+Q$ samples to simulate test scenarios. The $K+Q$ samples are further split into a support set containing $K$ samples to construct feature embeddings for classification and a query set containing $Q$ samples for model updating and evaluation. Therefore, FSED is usually solved with the so-called $N$-way-$K$-shot setting using meta-learning methods, among which metric-based meta-learning methods are the most popular, like prototypical networks~\cite{snell2017prototypical} and relation networks~\cite{hu2018relation}, in which distance metrics are used for classification.

\begin{figure}[t]
	\centering
	\subfloat[PA-CRF]{\label{fig:visual_a}\includegraphics[width=0.5\linewidth]{EMNLP 2022/figures/intro_vis_a.pdf}}
	\subfloat[HCL-TAT]{\label{fig:visual_b}\includegraphics[width=0.5\linewidth]{EMNLP 2022/figures/intro_vis_b.pdf}}\\	
	\caption{Visualization of triggers in the same episode on FewEvent test set. The left and right half shows support set representations without and with hybrid contrastive learning, respectively.}
	\label{fig:visual}
\end{figure}

Most works in FSED exploit metric-based meta-learning methods, in which the model needs to learn meta-knowledge from only a few instances in the \textit{support set} and generalize to predict labels for instances in the \textit{query set}. Specifically, in each episode, these methods first build a prototype for each class over the support set, then predict the labels for each instance in query set by matching with the closest prototype representation in the metric space. Indeed, many of these methods follow an identify-to-classify paradigm and are capable of keeping high generation on new event type based on a few observed samples~\cite{deng2020meta,lai2020exploiting,lai2020extensively}. However, the performance of such two-stage model is limited to the problem of error propagation caused by trigger misidentification. Thus, recent works formulate FSED as a few-shot sequence labeling task and apply Conditional Random Field based (CRF-based) methods to jointly identify and classify triggers. Nevertheless, it is usually challenging for these CRF-based methods to fully learn event type dependencies from a single sentence, since a sentence commonly contains only one trigger, or even worse with limited data in FSED. An example is presented in Figure~\ref{fig:visual_a}, even if the state-of-the-art method PA-CRF~\cite{cong2021PACRF} is powerful in exploring event type dependencies via Gaussian distribution for approximation, it is still incapable of generating well discriminative  representations for each event type in the whole embedding space.


%For better solutions, we seek to study the learning process of ED and explore the reason behind the lack of generalization. We argue that typical cross-entropy loss may not be the best choice for ED. As described by \cite{cao2019learning}, cross-entropy loss used in diverse classification tasks mainly focuses on minimizing the difference between predicted and ground-truth probability distributions rather than maximizing the margin between different classes, which may cause \textit{poor margin}, \ie the margin is too small for ambiguous instances near the decision boundary to give confident predictions. Poor margin leads to overlap between classes, which is the main reason for the lack of generalization. Intuitively, as illustrated in the left part of Figure~\ref{fig:poor_margin}, features learned by cross-entropy loss could be scattered in the latent space, resulting in poor margin and harming the performance.

Actually, it is non-trivial to solve the problem. Typical metric-based models are mostly optimized with a query-anchored cross-entropy loss based on the similarity between each query instance and all prototypes. However, we find that the gradient directions of prototypes are not always optimized very well during training, and may not guarantee the learnt representations of prototypes are discriminative via optimizing the query-anchored loss, which in turn harms the learning of query instances. Detailed proof can be found in Appendix~\ref{sec:D}.

To address the problem, in this paper, we propose a \textbf{\underline{H}}ybrid \textbf{\underline{C}}ontrastive \textbf{\underline{L}}earning (\textbf{HCL}) method to improve the representations for instances in both support set and query set. Specifically, we first propose a \textbf{\underline{S}}upport-\textbf{\underline{S}}upport \textbf{\underline{C}}ontrastive \textbf{\underline{L}}earning (\textbf{SSCL}) method to makes it prone to generating more discriminative representations of prototypes, via encouraging instances of the same type closer and others of different types farther away within support set. However, the optimization direction of SSCL is still unclear and only information within the support set is considered. Therefore, inspired by~\cite{gao2021contrastive}, we further design a \textbf{\underline{P}}rototype-\textbf{\underline{Q}}uery \textbf{\underline{C}}ontrastive \textbf{\underline{L}}earning (\textbf{PQCL}) method, which pulls query instances together with the prototype of the same type and pushes them apart from prototypes of different types. Logically, PQCL is capable of guiding the learning process of SSCL in a theoretically sound way, and such two contrastive learning losses are helpful for query-anchored loss to generate more discriminative representations for both the support set and the query set. 

Additionally, another serious problem for typical FSED is that most of the words in ED sentences are non-triggers, \ie they do not belong to any event type, called ``O'' type. The unbalanced nature influences the representation learning of triggers, and leads to representation overlap problem between triggers and non-triggers. To address this issue, we further design a \textbf{T}ask-\textbf{A}daptive \textbf{T}hreshold (\textbf{TAT}). Our key insight is that, if the similarity between a query instance and all event types are lower than the average similarity between query instances and ``O'' type, then it is most likely to be a non-trigger. Thus, in each episode, we take the average similarity between all query instances and the prototype of ``O'' type as the threshold to filter misidentified triggers. This threshold can be easily adapted to any episode and ensure the generalization ability. As illustrated in Figure~\ref{fig:visual_b}, by combining the above components, our \textbf{HCL-TAT} could learn more discriminative representations and make better predictions, thus boosting the performance.

%To improve the margin without relying on additional resources, inspired by supervised contrastive learning (SCL) in computer vision~\cite{NEURIPS2020_d89a66c7}, we propose to make full use of existing annotations and extend self-supervised contrastive learning into a fully-supervised setting. Intuitively, as illustrated in Figure~\ref{fig:poor_margin}, after training with supervised contrastive loss, representations of the same type should get closer while representations of different types should be pushed apart. The key challenge in SCL for ED is to eliminate the influence of non-triggers. Since ED is a token-level classification problem, non-triggers take up a large part and thus the number of triggers in each batch is limited, which is called \textbf{trigger sparsity}. This phenomenon makes it difficult for contrastive learning to solve poor margin for ED. To overcome trigger sparsity, we propose a \textbf{P}rototypical \textbf{C}ontrastive learning method for \textbf{E}vent \textbf{D}etection, namely \textbf{PCED}. Inspired by \cite{wang2021contrastive}, PCED exploits PLMs as the text encoder, and calculates prototypes for each event type through an average of instances. By encouraging representations of triggers to be closer to the prototype of the same type than other prototypes, the model could associate with all event types in the dataset, bringing more stable training and increasing the margin between types. Furthermore, to eliminate the influence of outliers for prototype representation, we iteratively select the most relevant instances and discard outliers of each type to update prototypes during training. Finally, since closer types in the latent space are more difficult to distinguish and thereby make more contribution to poor margin, we re-weight the contrastive loss according to the distance between prototypes to pay more attention to these hard cases.

%Specifically, we design a \textbf{P}rototypical \textbf{C}ontrastive learning method for \textbf{E}vent \textbf{D}etection, namely \textbf{PCED}, to bring more discriminative representations for ED. Our model consists of three components: (i) a text encoder using dynamic multi-pooling to obtain word representations; (ii) a prototypical contrastive learning module to make representations of the same event closer to the corresponding prototype and further away from other prototypes; (iii) a prototype adjustment module to dynamically update prototypes with the most representative instances and re-weight the contrastive loss concerning the relevance between event types.

The contributions of our work are summarized as follows:
\begin{itemize}
%
  \item We conduct the study of the limitation of query-anchored cross-entropy loss, namely, indistinguishability in embedding space, which harms the metric-based classification between query instances and prototypes.
  
  \item We propose a hybrid contrastive learning framework for the FSED task, which consists of two components, namely, SSCL and PQCL, to jointly improve the learning of instances on both the support set and the query set, which in return enhance the performance of FSED. Besides, we also propose a task-adaptive task-adaptive threshold (TAT) to eliminate the misidentification of trigger words.
%
  \item Experiments on FewEvent dataset in different settings demonstrate the advantages of our proposed HCL-TAT over various strong baseline methods.
\end{itemize} 

==> EMNLP 2022/sections/limitations.tex <==
\section*{Limitations}

In FewEvent, each sentence has exactly one trigger word, so the sampling process is simplified into randomly selecting sentences containing specific events, and in each episode, it's unlikely for instances of ``O'' type to belong to any other event type that is not inluded in the current episode. However, in real-world scenarios, a sentence may contains multiple trigger words, which could bring more complicated settings. For example, we have to consider that instances of ``O'' type might belong to other event types that are not sampled in this episode, and the contrastive loss should be modified to adapt for such scenarios.

Besides, due to the huge memory cost, we only make full use of provided data, and do not consider data augmentation in contrastive learning, which has been proved effective in previous contrastive learning works. We believe that by conducting data augmentation and introducing more self-supervised signals, the performance of FSED could be further improved, which is worth for future research. 

==> EMNLP 2022/sections/method.tex <==
\section{Methodology}

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\textwidth]{figures/model_camera_ready.pdf}
    \caption{Overall framework of the proposed HCL-TAT model. HCL-TAT is based on a prototypical network, composed of two components: (a) hybrid contrastive learning including support-support contrastive learning and prototype-query contrastive learning; (b) task-adaptive threshold based on the logits in each episode.} %It exploits external knowledge and label-enhanced meta-learning to improve both trigger identification and event classification, respectively.}
    \label{fig:model}
\end{figure*}

%In this section, we introduce the proposed KEPN-LS model, which exploits external knowledge to enhance the representations and develops a prototypical network with label semantics to solve the above-mentioned challenging. In general, the proposed KEPN-LS model contains two components, as illustrated in Figure \ref{figure_model}: (1) knowledge enhancement, which extracts and embeds event-related frames from sentences; (2) prototypical network, which constructs a few-shot event detection framework and further improves the performance with label semantics.

\subsection{Overview}
An overview of the proposed HCL-TAT method is illustrated in Figure~\ref{fig:model}. We first give the problem statement in Section~\ref{Sec: 3.2}, then introduce the backbone prototypical network in Section~\ref{Sec: 3.3}. In Section~\ref{Sec: 3.4} and Section~\ref{Sec: 3.5}, we detailedly describe the hybrid contrastive learning and task-adaptive threshold method respectively. Finally, the training process is given in Section~\ref{Sec: 3.6}.

%\subsection{Problem Definition}
%
%In this paper, the event detection task is divided into two stages: trigger identification and event classification. In trigger identification, we follow settings of traditional supervised learning. Given a sentence $s = \{w_1, w_2, ..., w_n\}$ of length $n$, the model needs to predict a label for each $w_i$, marked as trigger or non-trigger word.
%
%In event classification, the problem is defined with $N$-way-$K$-shot setting in meta-learning. Specifically, the model is given a support set with $N$ event types and one \textit{NONE} type. Each event type (including \textit{NONE} type) has only $K$ samples. Besides, there is also a query set which contains an unlabeled query instance. The goal of event classification model is to predict the label of query instance with only limited samples in support set.

\subsection{Problem Statement\label{Sec: 3.2}}

In this paper, we formulate few-shot event detection (FSED) as a few-shot sequence labeling task. Given a sentence $\mathcal{X}=\{x_1, x_2, ..., x_n\}$ composed of $n$ tokens and its corresponding label sequence $\mathcal{Y}=\{y_1, y_2, ..., y_n\}$, each token $x_i$ is categorized into an event type. Besides the defined event types in the dataset, we add an ``O'' type to denote for tokens that do not belong to any event type (called non-triggers). Then, FSED is defined with a typical $N$-way-$K$-shot setting. Specifically, given a support set $\mathcal{S}=\{\mathcal{X}^{(i)}, \mathcal{Y}^{(i)}\}_{i=1}^{N \times K}$ which has $N$ event types with $K$ labeled samples for each type, and a query set $\mathcal{Q}=\{\mathcal{X}^{(i)}, \mathcal{Y}^{(i)}\}_{i=1}^{N \times M}$ which has the same $N$ event types as $\mathcal{S}$ with $M$ samples for each type, we formulate a $N$-way-$K$-shot task or episode as $\mathcal{T}=\{\mathcal{S}, \mathcal{Q}\}$. Note that in each episode we also have an additional ``O'' type. The goal of FSED is to predict the labels for instances in $\mathcal{Q}$ based on $\mathcal{S}$. Specifically, in training stage, the classification results of $\mathcal{Q}$ are used to update model parameters, while in testing stage, the classification results are used to evaluate the model. The training phase is composed of a set of episodes $\mathcal{T}_{train}=\{\mathcal{T}_i\}_{i=1}^{M_{train}}$, and the testing phase is composed of another set of episodes $\mathcal{T}_{test}=\{\mathcal{T}_i\}_{i=1}^{M_{test}}$. $M_{train}$ and $M_{test}$ denote the number of training episodes and testing episodes respectively, and the label set of $\mathcal{T}_{train}$ and $\mathcal{T}_{test}$ are disjoint.


\subsection{Prototypical Network\label{Sec: 3.3}}

%这里要把基本的流程写完，从输入到编码到原型网络计算loss

Following~\citet{cong2021PACRF}, we select BERT as the text encoder to represent event mentions. We encode the sentence $\mathcal{X}$ into a sequence of hidden embeddings as follows,
\begin{equation}
    \label{equ:sentence_encoder}
    \{\vec{h}_1, \vec{h}_2, ..., \vec{h}_n\} = f(\mathcal{X},\theta),
\end{equation}
where $f(:,\theta)$ is the encoder and $\vec{h}_i$ is the hidden representation of each token $x_i$.

We then adopt the widely-used prototypical network (Proto)~\cite{snell2017prototypical} as our backbone, in which the classification results are obtained by matching instances with prototypes of each class in the metric space. During each episode, Proto first computes prototypes for each class $c$ by averaging instances in support set:
\begin{equation}
    \label{eq:proto_compute}
    \vec{p}_c = \frac{1}{K}\sum_{i \in \mathcal{S}(c)}\vec{h}_i, \;c=0,1,...,N,
\end{equation}
where $\vec{p}_i$ is the prototype for class $c$, $\mathcal{S}_{c}$ represents for all the words of class $c$ in $\mathcal{S}$. Then in training phase, the prototypes and query instances are fed into a non-parametric distance-based classifier to compute the cross-entropy loss for few-shot classification:
\begin{gather}
    \label{eq:ce_loss}
    \mathcal{L}_{CE} = -\sum_{(x_i,y_i) \in \mathcal{Q}}\operatorname{log}P(y_i|x_i,\mathcal{S}),\\
    P(y_i|x_i,\mathcal{S}) = \frac{\operatorname{exp}(-d(\vec{h}_i, \vec{p}_{y_i}))}{\sum_{c \in \mathcal{C}}\operatorname{exp}(-d(\vec{h}_i, \vec{p}_{c}))},
\end{gather}
where $\mathcal{C} = \{0,1,...,N\}$ denotes for the sampled class set including an additional ``O'' type, $d(\cdot)$ is a metric function to measure the similarity between query instances and prototypes.

We then analyze the bottleneck of query-anchored loss in Eq. (\ref{eq:ce_loss}). Assuming $d(\cdot)$ is dot product, $\vec{p}^{pos}$ represents for the prototype of class $y_i$ and $\vec{p}^{n}$ represents for any prototype of different classes, we compute the gradient \wrt $\vec{h}_i$, $\vec{p}^{n}$ and $\vec{p}^{pos}$ respectively:
\begin{gather}
    \frac{\partial \mathcal{L}_{CE}}{\partial \vec{h}_i} = \frac{\sum_{n}\Delta_n (\vec{p}^n - \vec{p}^{pos})}{1 + \sum_{n}\Delta_n},\\
    \frac{\partial \mathcal{L}_{CE}}{\partial \vec{p}^{n}} = \frac{\Delta_n \vec{h}_{i}}{1 + \sum_{n}\Delta_n},
    \frac{\partial \mathcal{L}_{CE}}{\partial \vec{p}^{pos}} = -\frac{\sum_{n}\Delta_n \vec{h}_{i}}{1 + \sum_{n}\Delta_n},\\
    \Delta_n = \operatorname{exp(\vec{h}_i \cdot \vec{p}^n - \vec{h}_i \cdot \vec{p}^{pos})}.
\end{gather}

We can conclude that the query instance $\vec{h}_i$ has a better update direction compared with prototypes, and this makes it hard to learn good representations for the prototypes, which could in turn affects the learning of $\vec{h}_i$, since the gradient \wrt $\vec{h}_i$ approaches to zero when $\vec{p}^{pos}$ and $\vec{p}^{n}$ are close in the embedding space. Therefore, we propose hybrid contrastive learning method to learn more discriminative representations and break this bottleneck. Proof details can be found in Appendix~\ref{sec:D}.


\subsection{Hybrid Contrastive Learning\label{Sec: 3.4}}

Hybrid contrastive learning (HCL) consists of two components: support-support contrastive learning (SSCL) applied to instances within $\mathcal{S}$ for more discriminative prototype representations and prototype-query contrastive learning (PQCL) applied between $\mathcal{S}$ and $\mathcal{Q}$ to guide the optimization process for instances in both set.

\subsubsection{Support-Support Contrastive Learning}

To produce better prototypes, we should learn more discriminative representations for instances in $\mathcal{S}$. Therefore, naturally we follow a supervised contrastive learning manner to construct our SSCL loss. We use label information to construct positive and negative pairs. In each episode, for word $x_i$, we take instances of its same class in $\mathcal{S}$ as positive pairs $\mathcal{P}(i)$ and instances of different classes in $\mathcal{S}$ as negative pairs $\mathcal{N}(i)$. Empirically, since a non-linear projection layer improves the representation quality for contrastive learning~\cite{chen2020simple}, we exploit a 2-layer MLP to project the token representations to a latent space.
\begin{equation}
    \label{projection_head}
    \tilde{\vec{h}}_i = \matrix{W}_2\sigma(\matrix{W}_1\vec{h}_i),
\end{equation}
where $\matrix{W}_1$ and $\matrix{W}_2$ are trainable weights, and $\sigma$ is an activation function.

We then encourage the positive pairs to pull closer and negative pairs to push further. In this way, we make instances in $\mathcal{S}$ more discriminative and produce more compact clusters to generate better prototypes. Specifically, we take dot product to measure the similarity between instances, and the SSCL loss is calculated as follows:
\begin{gather}
    \label{equ:SSCL_loss}
    \mathcal{L}_{SSCL} = \sum_{(x_i,y_i) \in \mathcal{S}}\mathcal{L}_{SSCL_{i}},\\
    \mathcal{L}_{SSCL_{i}} = -\operatorname{log}\frac{\operatorname{exp}(\tilde{\vec{h}}_i \cdot \tilde{\vec{h}}_j / \tau)}{\sum_{k \neq i}\operatorname{exp}(\tilde{\vec{h}}_i \cdot \tilde{\vec{h}}_k / \tau)},
\end{gather}
where $\tau$ is a scalar temperature parameter. In practice, we apply $\ell_2$ normalization to $\tilde{\vec{h}}_i$ for numerical stability.

\subsubsection{Prototype-Query Contrastive Learning}

By adopting SSCL, instances in the support set are enforced to be more separable. However, the optimization direction is still unclear without the guidance of query set. To this end, inspired by~\cite{gao2021contrastive}, we propose prototype-query contrastive learning (PQCL) to eliminate the gap. Similarly, we take each prototype as the anchor, and regard query instances of the same class as positive pairs and query instances of different classes as negative pairs. Given a class $c \in \mathcal{C}$, the positive pairs set and negative pairs set are defined as $\mathcal{Q}_{c}^{pos}$ and $\mathcal{Q}_{c}^{neg}$ respectively. The PQCL loss is calculated by:
\begin{gather}
    \label{equ:PQCL_loss}
    \mathcal{L}_{PQCL} = \sum_{c \in \mathcal{C}}\sum_{(x_i, y_i) \in \mathcal{Q}_{c}^{pos}}\mathcal{L}_{PQCL_{c}^{i}},\\
    \mathcal{L}_{PQCL_{c}^{i}} = -\operatorname{log}\frac{sim_{c}^{i}}{sim_{c}^{i} + \sum_{(x_k, y_k) \in \mathcal{Q}_{c}^{neg}}sim_{c}^{k}},\\
    sim_{c}^{i} = \operatorname{exp}(\vec{p}_{c} \cdot \tilde{\vec{h}}_i / \tau).
\end{gather}

We then combine the two contrastive losses as a hybrid contrastive learning (HCL) method, to produce more discriminative prototypes for query instances. Our HCL is complementary to the query-anchored cross-entropy loss $\mathcal{L}_{CE}$, and by optimizing the losses jointly, the model can obtain better representations for both support set and query set.

\subsection{Task-adaptive Threshold\label{Sec: 3.5}}

The proposed HCL could produce better representations for both support set and query set. However, since ``O'' type contains all instances that do not belong to any event type, the semantics of those instances are complex, making it hard to separate them even with the help of HCL. Therefore, it's important to further regularize the classification process for more accurate predictions. Naturally, we can set a threshold and let query instances whose similarity to all event types are lower than the threshold to output an ``O'' type prediction.

However, manually designed thresholds are hard to tune and lack generalization. Thus, based on the episodic training in FSED, we propose a task-adaptive threshold method. Intuitively, since the similarity between query instance and prototype can be regarded as a confidence score, in each episode, we take the average value of similarities between all query instances and ``O'' type as the threshold for automatically separating triggers and non-triggers. If the similarity between a query instance and an event type cannot even reach the calculated threshold, then it's unlikely for the query instance to be a trigger of that event type. We use probability to represent for similarity and the threshold $t$ can be defined as:
\begin{equation}
    \label{eq:threshold}
    t_{meta} = \frac{1}{|\mathcal{Q}|}\sum_{(x_i, y_i) \in \mathcal{Q}}P(y_i = 0 | x_i, \mathcal{S}).
\end{equation}

In this way, we could regularize the classification process by eliminating the misidentification of triggers.

\subsection{Training Process\label{Sec: 3.6}}

By combining the hybrid contrastive loss and task-adaptive threshold, we obtain the full method HCL-TAT. In each training episode, the model is optimized with the mixture of query-anchored cross-entropy loss and hybrid contrastive loss:
\begin{equation}
    \label{final_loss}
    \mathcal{L} = \mathcal{L}_{CE} + \alpha \mathcal{L}_{SSCL} + \beta \mathcal{L}_{PQCL},
\end{equation}
where $\alpha$ and $\beta$ are trade-off parameters to balance the losses. During training and testing phase, we both use the threshold to regularize the classification. Finally, we randomly select multiple testing episodes and report the mean result to evaluate the performance.


==> EMNLP 2022/sections/related_work.tex <==
\section{Related Work}

%Event detection has attracted extensive research interest. 

%
%\paratitle{Feature based ED}.
%Conventional ED approaches are usually on the
%basis of classical supervised learning models, \eg support vector machine (SVM),
%which heavily rely on well-designed handcrafted features (\eg relations among event mentions~\cite{liao2010using}, textual features \cite{ji2008refining})
%or language-specific resources (\eg lexical/syntactic features~\cite{ahn2006stages}). These methods achieve preliminary results based on rich features extracted from raw text, however, the performance highly relies on the quality of features, and it's hard to be fit for new domains since the feature design is domain-related.


\paratitle{Data-driven Event Detection.}
Early ED approaches rely on traditional machine learning models with handcrafted features to extract events \cite{ji2008refining,liao2010using}. With advances in deep learning, many research efforts have
been dedicated to enhancing ED with different neural network architectures
like \textbf{CNN-based} model~\cite{chen2015event,nguyen2016modeling} and \textbf{RNN-based} model~\cite{nguyen2016joint,feng2016language}. Recently, pre-trained language models (PLMs) are adopted to leverage rich information from large-scale corpora~\cite{yang-etal-2019-exploring,tong2020improving,lai-etal-2020-event}. These methods achieve promising results for supervised ED, but they could not adapt well to FSED with limited data.

\paratitle{Few-shot Event Detection.}
 In recent years, there have been several attempts to conduct meta-learning based approaches~\cite{snell2017prototypical,hu2018relation} for FSED. \citet{deng2020meta} proposed the benchmark FSED dataset FewEvent, and designs a dynamic-memory-based prototypical network (DMBPN) to preserve contextual information of event mentions. \citet{lai2020exploiting} and \citet{lai2020extensively} proposed intra and inter-cluster matching losses to provide more training signals. However, these works categorize events at sentence-level and are solely for the event classification task. Recently, \citet{cong2021PACRF} proposed to treat ED as few-shot sequence labeling task and solved with a modified PA-CRF model, but they still suffer from poor representation learning. In this paper, we propose to exploit contrastive learning to produce more discriminative representations.



\paratitle{Contrastive Learning.}
Contrastive learning has been widely used in various domains based on an idea to pull together similar instances and push apart distinct instances. \textbf{Self-supervised learning} designs specific strategies to generate positive and negative pairs from unsupervised data~\cite{chen2020simple,gao2021simcse,yan-etal-2021-consert,wang-etal-2021-cleve,mcclk2022,KGIC2022,wang2022multi}. As an extension, \textbf{supervised contrastive learning} which leverages label information to generate positive and negative pairs is further proposed~\cite{NEURIPS2020_d89a66c7,gunel2020supervised,wang2021contrastive}. Recently, contrastive learning is also used in few-shot learning tasks to improve the performance~\cite{gao2021contrastive}, by pulling query samples closer to the prototype of the same class and further away from those of different classes. In this paper, we propose a hybrid contrastive learning (HCL) method, composed of two complementary contrastive losses, to generate more discriminative representations for both support and query set. With the help of a task-adaptive threshold (TAT) method, the proposed HCL-TAT can fully make use of limited data and boosts the performance.


%Especially, in computer vision, contrastive learning based methods have achieved great success, by viewing differently augmented views of the same image as positive samples and introducing contrastive loss to maximize the agreement between different views. Recently, contrastive learning is extended to supervised settings by utilizing label information to construct positive and negative samples and achieve promising result in both supervised and semi-supervised scenarios.
%In the field of NLP, contrastive learning has also been used in numeral tasks, to generate more task-relevant sentence representations \cite{yan-etal-2021-consert}

%but mainly in self-supervised manners \cite{wang-etal-2021-cleve} or a simple supervised setting in low-resource scenarios \cite{gunel2020supervised}

%Although deep-learning based methods have achieved remarkable performance, most of such data-driven methods primarily rely upon supervised learning and require large-scale annotations, which may be easily prone to over-fitting (especially for unseen classes/instances) due to the the scarcity and imbalance natural of annotations. 
%
%Recently, meta-learning based approaches have gained great success in few-shot learning (FSL)~\cite{snell2017prototypical} tasks, which is capable of  learning  knowledge from a small number of samples and generalizes it to new classes (\aka ``learning-to-learn'').
%
%Therefore, there have been several attempts to conduct meta-learning based approaches for ED task. Deng \etal~\cite{deng2020meta} proposes to learn the prototype representation of each class via a dynamic-memory-based prototypical network, and then calculate the distances to different classes within a learnt metric space for event classification. Lai \etal~\cite{lai2020extensively} employ a matching network to learn the mapping between the labelled support set (as well as unlabelled examples) and their corresponding labels. However, the purpose of these studies are different from the current work (\ie event detection and  event classification), as they categorize events at sentence-level and are solely for the event classification task. Different from them, Cong \etal~\cite{cong2020fewshot} treats ED as few-shot sequence labeling task and devises a modified CRF model. We argue that CRF is not the best choice since label dependencies are not important in ED. In contrast, we concentrate on leveraging label semantics into prototype calculation, to generate better representations and improve the performance on both traditional scenarios and few-shot scenarios.






%Recently, meta-learning has been extensively studied, and proven successful in many applications. Meta-learning can be explained as "learn to learn", allowing model to learn knowledge from only a few of samples, leading to good generalization performance.

%\cite{deng2020meta} and \cite{lai2020extensively} develop approaches to address few-shot event detection. However, these methods only focus on sentences and fail to detect trigger words, which limit their performance. In this paper, we combine our label-enhanced meta-learning model with a novel trigger identification model to do event detection, without restriction to few-shot scenarios.




